Detecting Parkinson's Disease From an Online Speech-task

In this paper, we envision a web-based framework that can help anyone, anywhere around the world record a short speech task, and analyze the recorded data to screen for Parkinson's disease (PD). We collected data from 726 unique participants (262 PD, 38% female; 464 non-PD, 65% female; average age: 61) -- from all over the US and beyond. A small portion of the data was collected in a lab setting to compare quality. The participants were instructed to utter a popular pangram containing all the letters in the English alphabet "the quick brown fox jumps over the lazy dog..". We extracted both standard acoustic features (Mel Frequency Cepstral Coefficients (MFCC), jitter and shimmer variants) and deep learning based features from the speech data. Using these features, we trained several machine learning algorithms. We achieved 0.75 AUC (Area Under The Curve) performance on determining presence of self-reported Parkinson's disease by modeling the standard acoustic features through the XGBoost -- a gradient-boosted decision tree model. Further analysis reveal that the widely used MFCC features and a subset of previously validated dysphonia features designed for detecting Parkinson's from verbal phonation task (pronouncing 'ahh') contains the most distinct information. Our model performed equally well on data collected in controlled lab environment as well as 'in the wild' across different gender and age groups. Using this tool, we can collect data from almost anyone anywhere with a video/audio enabled device, contributing to equity and access in neurological care.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

==> demographic_images/Conclusion.tex <==
\section{Conclusion}
\textbf{This section will be deleted}
% Being able to utilize various voice assistant technologies that are in everyone’s homes and offices these days to characterize speech anomalies can not only lead us to finding out interesting speech patterns, but also it can be great effort in data collection and finding out how we can create a unified data collection process. A framework like ours deployed in these scenarios can be beneficial for individuals who cannot visit a doctor for whatever reason in finding out anomalies in their speech pattern. PD diagnosis in it’s beginning stages is difficult and hence this can be a good effort towards the direction of making people aware. For a concrete diagnosis, it is recommended to visit a neurologist or a trained individual to receive a holistic diagnosis and we think that our effort can further encourage that.
% \clearpage

\begin{enumerate}
    \item Number of Super-PARK data \SW{54}
    \item Total data, how many PD, how many Non-pd, no of male, female, etc \SW {Total: 726, PD: 262, NonPD: 464, Male: 325, Female: 401 }
    \item a age-distribution plot: say the buckets will be <30,30-40,40-50,50-60,60+. Within each bucket, please give the number of PD/Non-PD. I believe a bar-plot will be fine \VW{uploaded in SHAP}
    \item Sangwu: Two separate models for male/female and age>50 using max-little+PRAAT features
    \item Please make sure that demographic info in Table 1 is upt-to-date \VW{this is done}
    \item Sangwu: for the best model using all data and the MAX +PRAAT features, please report performance in two separate analysis: one for male and female and another for age<50 and age>=50. Please make sure to report all the confusion matrix derived metrics. \SW{Male (TN: 125, FP: 39, FN: 49, TP: 112), Female(TN:253, FP: 47, FN: 59, TP: 42) Old(TN: 316, FP: 78, FN: 102, TP: 149) }
    \item Victor and Sangwu: How many male, how many female? How many male have PD and non-pd, how many female have PD/Non-pd? \VW{PD Males: 161, Non-PD Males: 164, PD Females: 101, Non-PD Females: 300}
    
    \item Sangwu/Victor: There are some native English speaker and non-native. speaker in the dataset. Although we don't know who is a native speaker or not, country of residence can be a good proxy. Please report the main model's (with all data) confusion matrix scores for people who are native vs non-native. 
    
    \item Sangwu: Please give names to the axes in shap validation figure.

\end{enumerate}


==> sections/Background.tex <==
\section{Background}
\subsection{Parkinson's Diagnosis}
Parkinson’s is a neuro-degenerative disease, which affects the brain’s dopamine producing cells. As a result, patients show symptoms of tremor, rigidity, abnormal gait, random movement of hands, memory loss and many more \cite{kasper2005harrison,chou2017diagnosis}. Parkinson’s can additionally affect the muscles of the face, mouth and throat. A reduction in dopamine has been found to reduce respiratory muscle activation patterns \cite{solomon1993speech, vincken1984involvement}, and suppress the laryngeal muscles \cite{vincken1984involvement, baker1998thyroarytenoid}. Therefore, people with PD often exhibit symptoms of decreased loudness and softened speech \cite{ho1999speech}. Although there is no cure for Parkinson’s disease, there are therapies such as, Lee Silverman Voice Treatment (LSVT)\cite{el2002swallowing}, that can significantly improve the problems regarding voice and speech. However, in order to start a treatment, patients need to be diagnosed by an expert. In traditional setting, PD diagnosis is done using MDS-UPDRS \cite{goetz2008movement} -- a series of assessment tasks administered and observed by an expert. Currently, the assessment using the MDS-UPDRS is the gold standard. The expert makes the diagnosis as well as assess the severity by carefully observing the patient. Along with the motor symptoms, the expert listens to the free-flowing speech and engages in a conversation for speech symptoms. Then based on the softness of voice, clarity, an audibility a rating on a five point scale is given. In this paper, we used current advancements from audio processing and machine learning to automatically detect and characterize speech symptoms of Parkinson's disease.  

\subsection{Computer-based Systems for Detection of Parkinson's}

There have been various platforms and systems deployed to distinguish between PD and Non-PD. Wearable sensor data has been analyzed to detect movement cues \cite{Tzallas14, Lonini2018}. Non-invasive systems based on posed and spontaneous facial expressions have also been explored  \cite{bandini2017analysis, jacobs1995emotional, wu2014objectifying,tickle2004practitioners}, and smartphones have also been employed in analyzing PD \cite{arora2015detecting,Sahyoun11}. However, given the ubiquity, and ease of remote audio recording hardware, our work is focused on in the wild audio signal analysis. 

Researchers have looked into phonations from audio recordings \cite{arora2015detecting}, rhythm, stress and intonation \cite{playfer2008parkinson}.  Little et al. \cite{little2008suitability} introduced pitch period entropy as a measure of dysphonia to discriminate healthy people from people with PD. In a dataset from 31 people, a support vector machine using the dysphonia measure achieved a 91\% classification accuracy. Tsanas et al. \cite{tsanas2012novel} calculated 132 dysphonia measures from sustained vowels using four feature selection algorithms and two statistical classifiers. In a dataset of 263 samples from 43 individuals, authors have shown that the classifiers can achieve almost 99\% accuracy. The feature selection algorithms they used include, Least Absolute Shrinkage and Selection Operator (LASSO) \cite{tibshirani1996regression}, Minimum Redundancy Maximum Relevance (mRMR) \cite{peng2005feature}, RELIEF \cite{kira1992practical}, and Local Learning-Based Feature Selection (LLBFS)\cite{sun2009local}. The classifiers they used were random forests and support vector machine.  Peker et al. \cite{peker2015computer} presented a novel approach of using the mRMR feature selection technique combined with a complex-valued artificial neural network (CVANN) to detect PD from continuous phonation samples. They collected 195 biomedical sound measurements from 23 PD and 8 healthy subjects. Using their technique an accuracy of 98.12\% was achieved. V{\'a}squez-Correa et al. \cite{vasquez2015automatic} collected speech samples from 14 PD and 14 healthy subjects with a hand-held device in uncontrolled noise conditions. The features they used include the fundamental frequency of speech (F0), jitter, shimmer, log energy per window, and 12 MFCCs \cite{xu2004hmm}. Using a support vector machine and speech enhancement technique they obtained 86\% accuracy. Dubey et al. \cite{dubey2015echowear} designed a smartwatch based voice and speech monitoring system for people with PD receiving speech therapies from Speech-language pathologists. In a study with six participants, they found that their system performs close to a high-quality audio equipment in a speech laboratory. Rueda et al. \cite{rueda2017feature} analyzed features to detect PD from the continuous phonation of the vowel /a/. They identified a set of Mel-Frequency Cepstral Coefficient (MFCC) and Intrinsic Mode Functions (IMF) that can best represent the characteristics of PD. Along with the MFCCs and other hand-picked audio features, Vaiciukynas et al. \cite{vaiciukynas2017parkinson} used a convolutional neural network to detect PD from speech. In a study with 194 healthy controls and 74 PD participants they showed that segments of a sentence was better at predicting than the whole uttered sentence. Zhang et al. \cite{zhang2019pdvocal} presented a smart-phone based application -- PDVocal, which uses non-speech body sounds such as, breathing, clearing throat and swallowing as PD bio-marker. Using the features from non-speech sounds they were able to classify with more than 80\% accuracy. Zhan et al. \cite{zhan2016high} developed a smart-phone application -- HopkinsPD, to monitor the PD patients passively. They collected data from 121 PD and 105 controls over six month period. Using the random forest classifier they obtained 71\% accuracy discriminating treatment from baseline, where the conditions were medication sensitivity. Wroge, et al. applied various machine learning algorithms on a dataset \cite{bot2016mpower} (N=5826, PD<=1087) of participants saying "Aaaaaah" into their smartphones for as long as they can up to 10 seconds \cite{wroge2018parkinson}. They achieved highest accuracy of 86\% using Gradient Boosted Decision Tree (it should be noted, however, that 82\% of their data consisted of non-PD controls).

Although the current state of art has shown promising results, they have limitations such as small sample size \cite{vasquez2015automatic,little2008suitability,dubey2015echowear}, over sampling from the same participants \cite{peker2015computer}, noise-controlled data collection \cite{little2008suitability,rueda2017feature}, and age discrepancy between PD and control \cite{zhan2016high}. In this paper, we analyze the audio data that was collected in the wild, in uncontrolled noise condition. We compared our framework with the machine learning approaches that uses traditional audio features as well as hand crafted features.

==> sections/Introduction_legacy.tex <==
\section{Introduction}
%\MSI{Why should we consider Parkinson's disease seriously?}\\
%\MSI{Why early and remote detection is necessary?} \\
%\MSI{Why do we need a detection model that can be accessed by all?} \\
%\MSI{What has been done in this direction? Why speech analysis is popular?}\\

Access to good neurological care -- especially for Parkinson's -- is a rare privilege for millions of people around the world: especially in the developing countries. In 2013, there were 1200 neurologist in India for a population of 1.3 billion~\cite{khadilkar2013neurology}; average population per neurologist exceeds 3.3 million in Africa~\cite{howlett2014neurology}. On the other hand, 60,000 people  are diagnosed with Parkinson's disease every year in the US alone~\cite{pdIncidenceStat}, and similar patterns of rising PD cases -- -- fueled largely by the aging population -- can be seen across the globe. But the current projection of more than 12 million PD patients worldwide by 2040 is only part of the picture since more than 20\% PD patients remain undetected~\cite{schrag2002valid}. Early diagnosis and regular assessment are keys to ensure timely and appropriate medical intervention, which can improve the quality of life for a PD patient significantly.

A standard diagnosis requires the patient consulting a neurologist who administers a specific set of neurological tasks testing  speech, resting facial expression, finger tapping, and more. However, up-scaling the current neurological facilities to handle the deluge of PD patients is a daunting task.  
But, a web-based system that anyone with PD -- even from an under-served community -- can use on their phone/computer to perform some standard tasks and receive an assessment score denoting the severity of their tremors can help overcome the challenges significantly. Such a system will greatly increase  equity,  access  and inclusion in neurological care through providing critical service to millions of people around the world.

In this paper, we take a crucial step towards building such a system by designing a model that can detect PD/Non-PD from the speech task of pronouncing "the quick brown fox jumps over the lazy dog...”. Although automated PD detection has been researched through analyzing hand-movements~\cite{ali2020spatio}, movement pattern~\cite{Lonini2018}, or facial expressions~\cite{bandini2017analysis}, analyzing audio~\cite{little2008suitability,tsanas2012using,Arora2015,rueda2017feature} remains a promising avenue for PD detection. This is largely due to two important factors: around 90\% of PD patients exhibit vocal impairment~\cite{ho1998speech, logemann1978frequency} and this impairment is often one of the earliest indicators of PD~\cite{duffy2019motor}. 

Some of the most common voice disorders induced by PD are:
dysphonia (distortion or abnormality of voice), dysarthria (problems with speech articulation), and hypophonia (reduced voice volume). Two speech tasks are commonly used for detecting PD through exploiting the changing vocal pattern caused by these disorders: (i) sustained phonation (the subject is supposed to utter a single vowel for a long time with constant pitch), and (ii) running speech (the subject speaks a standard sentence, like “the quick brown fox jumps over the lazy dog”). Max et al.~\cite{little2008suitability} worked with automatic detection of dysphonia leading for classifying people with PD from the healthy ones. Tsanas et al.~\cite{tsanas2009accurate} focused on the telemonitoring of self-administered sustained vowel phonation task to predict the UPDRS rating~\cite{movement2003unified} -- a commonly used indicator for quantifying PD symptoms. These studies train their systems with data captured by advanced devices (e.g., wearable devices, high resolution video recorder, Intel AHTD telemonitoring system) that are not accessible by under-served people. The performance of these systems can reduce significantly when predicting on data collected in home acoustics, which can be amended through employing noise removal techniques~\cite{poorjam2019automatic}. Besides, completing the verbal phonation task correctly requires following a specified set of guidelines like completing the task in one breath -- which can be difficult for older subjects.

In contrast with the existing research, we analyze running speech task from the data collected through the parktest.net website. Our website can be accessed by anyone, anywhere in the world and requires only an internet connected device with integrated camera and microphone -- which is much more accessible and convenient for our target population. Besides,  modeling the running speech task provides certain advantages over modeling verbal phonation task: it does not require conforming to specific instructions, is more similar to the regular conversation, and therefore, the model can be potentially augmented to predict PD from regular conversation -- a potential game changer in PD assessment task. 

We collected speech recordings of 726 unique subjects (262 diagnosed with PD) through a website named ParkTest\footnote{https://parktest.net/}. We extract standard acoustic features like MFCC, Jitter variants, Shimmer variants, and pitch related features etc, and augment them with \textit{dysphonia features} designed to capture PD-induced vocal impairment~\cite{little2008suitability}. These features are modeled with machine learning algorithms like Support-Vector-Machine, Random Forest, LightGBM, and XGBoost to classify subjects with PD from the healthy ones. We trained additional models with features extracted from deep-learning based PASE encoder~\cite{Pascual2019} that represents the information contained in a raw audio instance through a list of encoded vectors.
Our contributions can be summarized as below:
\begin{itemize}
    \item We collected data from 726 unique subjects conducting the standard MDS-UPDRS tasks~\cite{goetz2008movement} -- modulating speech, facial expressions, and hand movements etc --  designed to assess PD. The data is largely collected from home environment, and therefore, well-suited for enabling automated PD assessment  for anyone, anywhere in the world in near future.
    \item We analyzed the speech task from that dataset to predict PD Vs Non-PD. Due to collecting data from home environment, the data is very noisy and posits a lot of different challenges: lower audio quality, incomplete compliance with the the instructions, background noise, variety in recording devices, etc.
    We have showed that our model can perform well in this noisy environment and can achieve  0.7533  AUC (Area Under The Curve) score on PD prediction task. The  AUC metric is calculated by varying the decision threshold of a model, plotting the ratio of True-positive-rate and False-positive-rate for each threshold, and calculating the area under the curve produced through the plotting. The AUC score of a random predictor is 0.5.
    
    \item We have deployed interpretation techniques to explain our model's decision making criteria and demonstrated that our model emphasizes on the previously well established MFCC features and a sub-set of dysphonia features that were proven to be  successful on the PD detection from verbal phonation task of pronouncing "AHHH"~\cite{little2008suitability,tsanas2012novel}.
    \item We also built specialized models for each of these three groups: Male, Female and Age-matched (constructed by removing subjects aged below 50) and showed that they also perform largely in par with the main model.
\end{itemize}






 

% \MSI{This may be a good place to discuss a bit about the interpretability of our model. Also, we need to discuss about the effect of removing lab-environment data -- our model retains similar performance even if we only use the completely self-supervised home-environment data. Also, the significance of SHAP values, and our interesting findings.}

% To the best of our knowledge, we are the first to analyze the self-supervised running speech task in the wild. Although such a task is very challenging, we are encouraging it because the running speech task is very similar to regular conversation. If a model can be trained to do well in this task, there remains a good possibility of detecting PD from regular conversation, which would be much more helpful, especially for the people who find it difficult to follow instructions. In this regard, our model looks promising, by achieving \textbf{0.7533 AUC} (the AUC of a random predictor is 0.5). We hope, this work will inspire contributions from the researchers towards developing a remote system for detecting Parkinson's disease, easily accessible by any person in the world.
%The distributions of age for the subjects of both categories (PD, non-PD) are similar (see Figure \ref{fig:age_pd_noon_pd_plot}).

%\MSI{More questions to be answered:}\\
%A reduction in dopamine has been found to reduce respiratory muscle activation patterns \cite{solomon1993speech, vincken1984involvement}, and suppress the laryngeal muscles \cite{vincken1984involvement, baker1998thyroarytenoid}. Therefore, people with PD often exhibit symptoms of decreased loudness and softened speech \cite{ho1999speech}. Although there is no cure for Parkinson’s disease, there are therapies such as, Lee Silverman Voice Treatment (LSVT)\cite{el2002swallowing}, that can significantly improve the problems regarding voice and speech. However, in order to start a treatment, patients need to be diagnosed by an expert. In traditional setting, PD diagnosis is done using MDS-UPDRS \cite{goetz2008movement} -- a series of assessment tasks administered and observed by an expert. Currently, the assessment using the MDS-UPDRS is the gold standard. The expert makes the diagnosis as well as assess the severity by carefully observing the patient. Along with the motor symptoms, the expert listens to the free-flowing speech and engages in a conversation for speech symptoms. Then based on the softness of voice, clarity, an audibility a rating on a five point scale is given. In this paper, we used current advancements from audio processing and machine learning to automatically detect and characterize speech symptoms of Parkinson's disease.
%5. What are we doing? Why processing wild data is more challenging?\\
%6. What is our uniqueness? \\
%7. How can any people benefit from our model? How can our model assist treatment/monitoring of PD patients'? \\
%8. Address our weakness and state that this is a baby step towards a robust detection system, that can be freely accessible by all people. \\
%8. What are the main contributions of this paper? \\
%As we experience a revolution in the ubiquity of voice computing through the forms of Amazon Alexa, Google Assistant/Home, and Siri, we are working towards a Parkinson's Disease risk assessment framework as simple as a person conducting a short oral test with their virtual assistant. While laboratory-based approaches of detecting Parkinson's Disease from audio recordings have been investigated [cite], fewer studies have focused on in the wild data. A system which works in the wild has to deal with numerous difficulties. For example, different users may have vastly differing audio acoustics in their home environments, there is a lack of uniformity in the devices, and multiple audio source can coincide. A computer based online system is likely to need to work with a wide variety of microphone hardware across a large international user base. In this paper, we present our analysis of audio data collected through an online interface. We show the algorithms we applied to detect Parkinson's disease and how these algorithms can reveal information about the features present in the data. Such an approach is not only scalable, but also avoids use of techniques which can not be extended to noisy in the wild data. 


%\MSI{Wasif's comments:}
%1. It is difficult to get Ahh data properly without prior training. Our examination of PARK reveals that. the data we are collecting can be done properly by people without prior knowledge of it as it is just a pseudo-natural conversation.
%2. Our data is more aligned towards natural conversation,. Although it is scripted, it still has data about every phoneme since we are using a pangram. so, it is one step towards analyzing natural conversation
%3. It opens up the possibllity of using this info in speech therapy if say we know that which parts of speech or phoneme are most distorted and so on.
% However, even with the scalability of an online framework, and the prevalence of Parkinson's Disease, there is still a lack of large data sets which would allow the direct application of state of the art deep learning algorithms. In this paper, we investigate a novel approach of leveraging transfer learning from the visual domain, and applying it to the speech domain. Large visual recognition networks pretrained on millions of images are used to detect visual cues in two dimensional audio spectograms of participant's speech samples. In summary, our study:
% \begin{itemize}
% \item provides a framework for remotely analyzing Parkinson's Disease risk by: i) prompting and recording individuals to read a phoneme-diverse phrase through a web application, ii) converting the audio into a mel-frequency spectrum image; iii) further training a pre-trained deep image classifier to assess the probability that an audio recording was recorded from someone with Parkinson's Disease;

% \item identifies that individuals with Parkinson's Disease have statistically significant difference in repeated word duration variance and mel-spectrum variance

% \end{itemize}







% Parkinson’s disease (PD) is the second most common neurodegenerative disease~\cite{de2000prevalence}, with an estimate of more than one million people in North America alone to be affected~\cite{lang1998medical}. Sadly, there is no cure for such a prevalent disease, but medication can alleviate the symptoms significantly if the patient is diagnosed early~\cite{singh2007advances}. A standard diagnosis requires the patient consulting a neurologist who administers a specific set of tasks involving speech, movement, and other mental and physical activities. However, not every people has access to a neurologist. According to a study of 2013~\cite{khadilkar2013neurology}, there were only 1,200 neurologists in India, for a population of nearly 1.3 billion. More than 20\% PD patients remain undetected~\cite{schrag2002valid}, and thereby cannot be treated. Imagine the scenario, where any person can be diagnosed for PD right away, just by visiting a website. In this paper, we make a small step towards a remote system for PD diagnosis with a focus of making it accessible to any person in the world.

%Parkinson’s disease (PD) is a neurodegenerative disease, which affects the brain’s dopamine-producing cells. As a result, patients show symptoms of tremor, rigidity, abnormal gait, random movement of hands, memory loss, and many more that adversely affect their daily life\cite{kasper2005harrison,chou2017diagnosis}. It is the second most common neurodegenerative disease~\cite{de2000prevalence}, with an estimate of more than one million people in North America alone to be affected~\cite{lang1998medical}. Sadly, there is no cure for such a prevalent disease, but medication can alleviate the symptoms significantly if the patient is diagnosed early~\cite{singh2007advances}. A standard diagnosis requires the patient consulting a neurologist who administers a specific set of tasks involving speech, movement, and other mental and physical activities. However, not every people has access to a neurologist. According to a study of 2013~\cite{khadilkar2013neurology}, there were only 1,200 neurologists in India, for a population of nearly 1.3 billion. Also, it is extremely difficult for a person living in rural area to consult a neurologist. As a result, more than 20\% PD patients remain undetected~\cite{schrag2002valid}, and thereby cannot be treated.





% Every nine minutes, one person in the United States is diagnosed with Parkinson's Disease (PD) -- the fastest growing neurological disorder in the world with over 10 million confirmed diagnosis. A standard diagnosis requires the patient consulting a neurologist who administers a specific set of neurological tasks testing  speech, resting facial expression, finger tapping, and more. However, access to a neurologist is a rare privilege for many people around the world: in 2013, there were 1200 neurologist in India for a population of 1.3 billion~\cite{khadilkar2013neurology}. Due to lack of facilities, more than 20\% of PD patients remain undiagnosed~\cite{schrag2002valid}. Often the people who get diagnosed are at an advanced stage of PD progression, rendering the standard treatment ineffective. Even the patients who get diagnosed often face difficulty in visiting a neurologists regularly due to lack of facilities nearby and decreased mobility induced by PD; 40\% of PD patients over age 65 do not visit a neurologist regularly~\cite{langevin2019park}. 





% Due to the ubiquity of electronic devices, Internet, and advancement in technology, researchers are focusing on detecting the symptoms of PD remotely. Recent studies show that, symptoms involving speech and motor functions can be detected with clinical accuracy using statistical regression and machine learning techniques~\cite{Arora2015, rueda2017feature, little2008suitability}. Wearable sensor data has been analyzed to detect movement cues \cite{Tzallas14, Lonini2018}. Non-invasive systems based on posed and spontaneous facial expressions have also been explored  \cite{bandini2017analysis, jacobs1995emotional, wu2014objectifying,tickle2004practitioners}. While researchers are trying to detect PD based on multitude of remote tasks, significant progress has been made in speech-related tasks because of the ubiquity of audio recording hardware and ease of performing these tasks. Also, studies report that around 90\% of PD patients exhibit vocal impairment~\cite{ho1998speech, logemann1978frequency} and it can be one of the earliest indicators of PD~\cite{duffy2019motor}.

==> sections/alt-abstract.tex <==
Despite being a prevalent disease, diagnosis for Parkinson's Disease (PD) is still inaccessible to most of the people. Although there has been studies on detecting PD remotely, these studies use data collected using advanced devices and sometimes under supervision of experts, which does not generalize well for unsupervised home environment. In this paper, we envision a web-based tool that can help anyone, anywhere around the world to screen for Parkinson's Disease (PD) by merely recording a short speech task in home acoustics. We collected data from 726 unique subjects (262 with PD and 464 Non-PD) -- from all over the US and beyond -- uttering the sentences ``the quick brown fox jumps over the lazy dog $\cdots$''. We extracted both interpretable acoustic features (like MFCC, Jitter and Shimmer variants) and deep learning based features from the speech data and trained several machine learning models on them. The best model XGBoost achieved 0.75 AUC (Area Under The Curve) performance on determining presence of Parkinson's by modeling the standard acoustic features. The prediction is mostly impacted by the widely used MFCC features and a subset of previously validated dysphonia features leading to detecting Parkinson's. A further analysis for gender and age-restricted groups show that our model performs well across these groups as well. Our proposed model can potentially be used anywhere by anyone, contributing to health equity, access and inclusiveness in neurological care, specially among the under-served people around the world.

==> sections/figure_latex/female_model_shap_weight.tex <==
% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/MAX_PRAAT_Female_LGBM_Bar.png}
%     \caption{Female model Shap Absolute value}
%     \label{fig:female_model_shap_absolute}
% \end{figure}


% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/MAX_PRAAT_Female_LGBM.png}
%     \caption{Female model Shap real value}
%     \label{fig:female_model_shap_real_number}
% \end{figure}



\begin{figure}
    \centering
    % \subfigure[]{\includegraphics[width=\linewidth]{SHAP/MAX_PRAAT_Female_LGBM_Bar.png}} 
    % \subfigure[]{\includegraphics[width=\linewidth]{SHAP/MAX_PRAAT_Female_LGBM.png}} 
    \includegraphics[width=\linewidth]{SHAP/MAX_PRAAT_Female_LGBM.png}
\caption{\textit{SHAP for Female model:} The most impactful features are usually the MFCC features : mean MFCC values in each channel is represented by the prefix cepm and the variation in those channels by cepj. Apart from that features like RPDE (measuring uncertainty in F0 estimation), HNR (Harnomic to noise ratio ), ashr (median in amplitude perturbation), relative-band-power features (realbandpower1 and relbandpower3 (amount of power in the frequency range 0.5-1kHz and 2kHz-4kHz) also impact the model's behaviour. Besides, there are some influence from the Pitch related features as well (f0m,f0jr,f0std). Please refer to Table \ref{tab:feature_names} for a complete list of features and ~\ref{ssec:std_acoustic_feats} for a detailed description of features.}
    \label{fig:female_model_shap}
\end{figure}

==> sections/figure_latex/local_shap_analysis.tex <==
\begin{figure}
    % \centering
    \includegraphics[width=\linewidth]{SHAP/individual_plots/realPDpredPD.png}
\caption{SHAP analysis of an individual subject. The subject is a PD patient and the model correctly identified him as such. In the plot, the features colored in red are pushing the model towards predicting  the subject to be a PD patient. Conversely, the blue colored features are pushing the model towards predicting the subject as a Non-PD patient. The associated meaning with each feature's name is outlined in Table ~\ref{tab:feature_names}.
    % \textcolor{red}{higher value/lower value correctly used?}
    }
    \label{fig:real_pd_pred_pd}
\end{figure}


% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/individual_plots/realPDpredNonPD.png}
%     \caption{Real PD-> pred non-PD}
%     \label{fig:real_pd_pred_non_pd}
% \end{figure}


% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/individual_plots/realNonPDpredPD.png}
%     \caption{Real Non-PD-> pred PD}
%     \label{fig:real_non_pd_pred_pd}
% \end{figure}


% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/individual_plots/realNonPDpredNonPD.png}
%     \caption{Real Non-PD-> pred non-PD}
%     \label{fig:real_non_pd_pred_non_pd}
% \end{figure}

==> sections/figure_latex/old_people_model_shap_weight.tex <==
% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/MAX_PRAAT_Age_SVC_Bar.png}
%     \caption{Old people model Shap Absolute value}
%     \label{fig:old_people_model_shap_absolute}
% \end{figure}


% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/MAX_PRAAT_Age_SVC_Feature.png}
%     \caption{Old people model Shap real value}
%     \label{fig:old_people_model_shap_real_number}
% \end{figure}



\begin{figure}
    \centering
    % \subfigure[]{\includegraphics[width=\linewidth]{SHAP/MAX_PRAAT_Age_SVC_Bar.png}} 
    % \subfigure[]{\includegraphics[width=\linewidth]{SHAP/MAX_PRAAT_Age_SVC_Feature.png}} 
    \includegraphics[width=\linewidth]{SHAP/MAX_PRAAT_Age_SVC_Feature.png}
    \caption{\textit{SHAP for Age-matched model:} This figure depicts the most important features for the model using the Age-matched data. As before, the model is greatly influenced by dysphonia features (RPDE and PPE), MFCC features (prefixed cepm and cepj). Besides, there are notable influence from the Pitch related features (meanF0Hz,f0j,f0std) as well. Apart from that, features like HNR (Harnomic to noise ratio), ashr (median in amplitude perturbation), relative-band-power features (realbandpower1 ,relabandpower2 and relbandpower3) also impact the model's behaviour.  Please refer to Table \ref{tab:feature_names} foor a complete list of features and ~\ref{ssec:std_acoustic_feats} for a detailed description of features.}
    \label{fig:old_people_model_shap}
\end{figure}

\MSI{SHAP figures can be combined into one, or just keep one in the main paper and move the rest to supplementary materials. Also captions can be made shorter.}

==> sections/figure_latex/shap_weight.tex <==
% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/MAX-PRAAT_Bar.png}
%     \caption{Shap Absolute value}
%     \label{fig:shap_absolute}
% \end{figure}


% \begin{figure}
%     % \centering
%     \includegraphics[width=0.5\textwidth]{SHAP/MAX-PRAAT_feature.png}
%     \caption{Shap real value}
%     \label{fig:shap_real_number}
% \end{figure}
% The performance of various machine learning algorithms sing  the Standard-features and Embedding-features on the dataset that combines data from both Home-environment and Lab-environment. We can see that the models using Standard-features perform better than their Embedding-features using counterparts in terms of both Binary Accuracy and AUC. Although the model's perform similarly in using the Standard-features, XGBoost outperforms others by considering both the AUC and Accuracy metrics

\begin{figure}
    \centering
   
    \includegraphics[width=\linewidth]{SHAP/MAX-PRAAT_feature.png}
    %  \subfigure[]{\includegraphics[width=\linewidth]{SHAP/MAX-PRAAT_Bar.png}} 
    \caption{SHAP analysis of our model on all data: this figure depicts the most important features for a model by plotting the SHAP values of every feature in every data sample. Plot (a) arranges the features in two steps: (i) Sorts features by the mean of absolute SHAP value  over all samples, (ii) Uses SHAP values to show a distribution of how each feature impacts the model's output: red color represents high value of a feature, blue represents low. For example, higher values of the feature cepm3 (the second to last one) increases the model's output value. We see that the most salient features are usually the MFCC features : mean MFCC values in each channel is represented by the prefix cepm and the variation in those channels by cepj. Apart from that, features like RPDE (measuring uncertainty in F0 estimation), PPE (measure of inability of maintaining a constant F0), HNR (Harnomic to noise ratio), ashr (median in amplitude perturbation), realbandpower1 (amount of power in the frequency range 0.5-1kHz) also impact the model's behaviour significantly. 
    % \MSI{The caption is too long. Can we summarize a bit?}
    }
    \label{fig:shap_full_model}
\end{figure}



==> sections/figure_latex/three_figure_shap.tex <==
\begin{figure*}
    \centering
   
    \includegraphics[width=\textwidth]{SHAP/three_shap_combined.pdf}
    %  \subfigure[]{\includegraphics[width=\linewidth]{SHAP/MAX-PRAAT_Bar.png}} 
    \caption{The three figures above depict SHAP analysis of our best performing models on three separate datasets:(A) All data present; (B) Female data only; (C) Age-matched dataset (all subjects are above age 50). The figure depict the twenty most important features for a model in two steps: (i) Sorts features by the mean of absolute SHAP value  over all samples, (ii) Uses SHAP values to show a distribution of how each feature impacts the model's output: red color represents high value of a feature, blue represents low (notice the rightmost part of the figure). The MFCC related features are put within a red box fr increased visibility. Please refer to Table \ref{tab:feature_names} for a complete list of features and ~\ref{ssec:std_acoustic_feats} for a detailed description of features. In \textit{A.SHAP for Main-Model},  the most salient features are usually the MFCC features : mean and variation of MFCC values  in  $i$th channel is represented by MeanMFCC$i$ and VariationMFCC$i$ respectively. Apart from that, features like RPDE (measuring uncertainty in F0 estimation), PPE (measure of inability of maintaining a constant F0), HNR (Harnomic to noise ratio), MedianShimmer (median in amplitude perturbation), RealBandPower1 (amount of power in the frequency range 0.5-1kHz) also impact the model's behaviour significantly. In Part \textit{B.SHAP for Female model:} The most impactful features are usually the MFCC features as well. Apart from that features like RPDE (measuring uncertainty in F0 estimation), HNR (Harnomic to noise ratio ), MedianShimmer (median in amplitude perturbation), relative-band-power features (RealBandPower1 and RelBandPower3 (amount of power in the frequency range 0.5-1kHz and 2kHz-4kHz) also impact the model's behaviour. Besides, there are some influence from the Pitch related features as well (MedianPitch,MedianJitter,StdDevPitch). In \textit{C.SHAP for Age-matched model:}, the model is greatly influenced by dysphonia features (RPDE and PPE), MFCC features . Besides, there are notable influence from the Pitch related features (MeanPitch,MeanJitter,StdDevPitch) as well. Apart from that, features like HNR (Harnomic to noise ratio), MedianShimmer (median in amplitude perturbation), relative-band-power features (RelBandPower1 ,RelBandPower2 and RelBandPower3) also impact the model's behaviour.  
    }
    \label{fig:shap_three_models}
\end{figure*}


==> sections/intro-backup.tex <==
\section{Introduction}
As we experience a revolution in the ubiquity of voice computing through the forms of Amazon Alexa, Google Assistant/Home, and Siri, we are working towards a Parkinson's Disease risk assessment framework as simple as a person conducting a short oral test with their virtual assistant. While laboratory-based approaches of detecting Parkinson's Disease from audio recordings have been investigated [cite], fewer studies have focused on in the wild data. A system which works in the wild has to deal with numerous difficulties. For example, different users may have vastly differing audio acoustics in their home environments, there is a lack of uniformity in the devices, and multiple audio source can coincide. A computer based online system is likely to need to work with a wide variety of microphone hardware across a large international user base. In this paper, we present our analysis of audio data collected through an online interface. We show the algorithms we applied to detect Parkinson's disease and how these algorithms can reveal information about the features present in the data. Such an approach is not only scalable, but also avoids use of techniques which can not be extended to noisy in the wild data. 



% However, even with the scalability of an online framework, and the prevalence of Parkinson's Disease, there is still a lack of large data sets which would allow the direct application of state of the art deep learning algorithms. In this paper, we investigate a novel approach of leveraging transfer learning from the visual domain, and applying it to the speech domain. Large visual recognition networks pretrained on millions of images are used to detect visual cues in two dimensional audio spectograms of participant's speech samples. In summary, our study:
% \begin{itemize}
% \item provides a framework for remotely analyzing Parkinson's Disease risk by: i) prompting and recording individuals to read a phoneme-diverse phrase through a web application, ii) converting the audio into a mel-frequency spectrum image; iii) further training a pre-trained deep image classifier to assess the probability that an audio recording was recorded from someone with Parkinson's Disease;

% \item identifies that individuals with Parkinson's Disease have statistically significant difference in repeated word duration variance and mel-spectrum variance

% \end{itemize}

==> sections/limitations_written_by_Abdullah.tex <==

This paper recognizes all the limitations that have already been discussed in \cite{langevin2019park}. Since this tool is still at the level of academic research we aren't able to engineer it in a fashion to not rely on already available open source resources, that makes it easier to deploy it faster. At the time of writing this, our framework does not work for people with severe upper body disabilities or very late stages cognitive disabilities; for both cases there has to be someone present at all times to help them with doing these tasks and directing them what to do. One of the difficulties we faced during our analyzing phase is dealing with noise in the data. Other than environmental noise there are a lot of silences in the beginning and end of each audio file. While the solution for that might seem like trimming the silences using functions available through PRAAT or Librosa, in reality it's much more difficult than that. These libraries generally do the silence trimming based on decibel level so they are really looking for true silences, whereas in our data there's always something going on that registers beyond those decibels, hence arbitrarily choosing a number would only result in data loss as we won't be able to generalize it. Since we have to age-match the data we have to keep in mind that a lot of this older population aren't necessarily as comfortable with computers compared to their younger counterparts regardless of how user friendly and accessible the it is made for them, which only adds to the difficulties of an already difficult problem. Other than that we also cannot ensure hardware similarity across all data points. What we mean by that is different people at their homes are using different computer of different brand, model and age. The way this complicates our problem is that all these different computers use different kinds of mics and sometimes different kinds of webcams which also can have different forms of audio input, and if the computer is old then it will have poorer hardware quality as well. Because of this reason we cannot also just choose to get rid of certain frequencies to remove noise, which we have noticed while curating our data.

There are various aspects of this specific domain of Parkinson's research that leave us wanting to look into more. Majority of the participants in our PD population are white. Since we first deployed this framework in the United States where majority of the population is white, this was something beyond our control to bring in more diverse data. It would be interesting to see how audio features and energy bands change across different races of people with PD. Other than that 92.5\% of the population speak English which leaves us wanting to know how these features would change across languages. We think that audio features may behave the somewhat similar way but temporal features would certainly be very interesting since we would have to design the sentences appropriate for the specific language where contextually it makes sense, we would have to keep in mind about using easier vs. more difficult pronouncing word and it would become even more interesting in languages that are deemed to be hard to speak in general. Since we have experimented with mel-spectrograms we are curious how deep learning approach would scale with other languages as well.

In this paper we have only analyzed two of the 17 tasks that are currently present: Task1 and Task6. As mentioned before, some of the other tasks consist of pronouncing more vowel sounds and reciting sentences. We would like to see what kind of audio differences are present there. Since this paper deals with mostly audio analysis we aren't able to expand our scope into all the rich video data we collect where participants are doing movement and expression related tasks. Even in the audio focused tasks, we aren't yet looking into how the facial expression changes. We have observed that when the PD participants are trying to focus on the computer screen to read the sentence they are not so aware about how their lips and jaw aren't necessarily in the most neutral position, which is a very interesting feature since it doesn't happen with Non-PD population. Other than that at different stages of PD people are also not able to keep their head completely still and there's always some kind of micro movement going on in a pattern which is not noticeable in Non-PD group. We think these would be a great avenue to explore in our future efforts.

==> sections/supplementary_materials.tex <==
\subsection{Predicting PD from Home-environment data only}


\input{sections/tables/super_park_not_in_test}
\MSI{Instead of creating subsubsections, we can briefly summarize the effects of removing lab-environment data.}
\subsubsection{Removing Lab-environment data from Test set}
In Table ~\ref{tab:res_super_park_not_in_test}, we present the results on Home-environment data by removing the  Lab-environment data from test set. As we are using leave-one-out-cross-validation, we have predictions on every data instance. We can see that the results exhibit almost the same pattern as in Table ~\ref{tab:res_with_super_park}. We are still getting the best performance using the Acoustic-features and the various models are performing almost the same. However, note that the test set of Table ~\ref{tab:res_with_super_park} and Table ~\ref{tab:res_super_park_not_in_training}  are not the same,hence the results are not directly comparable. But the results demonstrate that our models' performance do not get worse by excluding the Lab-environment data from test-set.








\subsection{Gender and age Stratified Analysis}


\subsubsection{Our Model's performance on Gender-stratified and age matched test-set}
\input{sections/tables/complete_model_but_gender_age_acoustic_metrics}

We separately analyzed the performance of our models trained on Acoustic-features presented in Table ~\ref{tab:res_with_super_park} on three different data-sets: Male subjects, Female subjects and Age-matched subjects -- created by removing all subjects below the age of 50. The result is presented in Table ~\ref{tab:complete_model_gender_age_stratified}. We would like to reiterate that we did not train any model for this purpose. We just analyzed how our previous models are working on different population groups. 
% As we employed leave-one-out cross validation, each data-point is put in the test set once. Therefore, we have prediction for all data-points.

From Table ~\ref{tab:complete_model_gender_age_stratified}, we can see that the best model's in each of Male and Age-matched domains have similar or better performance to the overall model's mentioned in Table~\ref{tab:res_with_super_park} in terms of AUC. However, the model performs worse for Female subjects in comparison to all subjects. As we can see from the demographics information in Table. ~\ref{tab:demography}, females are over-represented in the Non-PD group and under-represented in the PD group. Previous Epidemiological studies have shown that both incidence and prevalence of PD are 1.5–2 times higher in men than in women~\cite{van2003incidence,haaxma2007gender}. Therefore, we are more likely to get PD data-samples from male than female. To improve our model's performance, we plan to include more female PD subjects in our dataset in future. 



==> sections/tables/complete_model_but_gender_age_acoustic_metrics.tex <==
\begin{table*}

 \caption{Group-Specific-Performance: These scores are achieved after training the model on entire dataset and then checking the performance of the model on three separate groups: Male, Female and Age-matched. Age-matched group is constructed from people over 50 years old. We can see that the performance for each sub-group is in par with the performance on the entire dataset (Table ~\ref{tab:res_with_super_park}), except for the Female group. This performance degradation can be attributed to the PD/Non-PD imbalance within the Female group (101 PD Vs. 300 Non-PD) }
  \label{tab:complete_model_gender_age_stratified}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Algorithm     & \multicolumn{2}{l|}{Male} & \multicolumn{2}{l|}{Female} & \multicolumn{2}{l|}{Age-matched} \\ \hline
              & AUC        & Accuracy     & AUC         & Accuracy      & AUC        & Accuracy    \\ \hline
SVM           & \textbf{0.7751}     & \textbf{0.7292}       & 0.6741      & 0.7556        & \textbf{0.7543}     & \textbf{0.7209}      \\ \hline
Random Forest & 0.7554     & 0.7262       & 0.6893      & 0.7606        & 0.7466     & 0.7209      \\ \hline
LightGBM      & 0.7461     & 0.6892       & \textbf{0.7238}      & \textbf{0.7456}        & 0.752      & 0.7039      \\ \hline
XGBoost       & 0.7549     & 0.72         & 0.7127      & 0.7581        & 0.7421     & 0.7225      \\ \hline
\end{tabular}
\end{table*}

==> sections/tables/complete_model_but_super_park_gender_age_PASE_metrics.tex <==
\begin{table}[PASE]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Algorithm     & \multicolumn{2}{l|}{Male} & \multicolumn{2}{l|}{Female} & \multicolumn{2}{l|}{Old} \\ \hline
              & AUC        & Accuracy     & AUC         & Accuracy      & AUC        & Accuracy    \\ \hline
SVM           & 0.7511     & 0.6985       & 0.6862      & 0.7182        & 0.735      & 0.6915      \\ \hline
Random Forest & 0.7049     & 0.6492       & 0.6807      & 0.7282        & 0.7123     & 0.6837      \\ \hline
LightGBM      & 0.7254     & 0.6646       & 0.7047      & 0.7282        & 0.7339     & 0.6791      \\ \hline
XGBoost       & 0.713      & 0.6708       & 0.6937      & 0.7082        & 0.7281     & 0.6806      \\ \hline
\end{tabular}
\end{table}

==> sections/tables/stratified_analysis_PASE.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Algorithm     & \multicolumn{2}{l|}{Male} & \multicolumn{2}{l|}{Female} & \multicolumn{2}{l|}{Old} \\ \hline
              & AUC        & Accuracy     & AUC         & Accuracy      & AUC        & Accuracy    \\ \hline
SVM           & 0.7402     & 0.68         & 0.675       & 0.7556        & 0.7285     & 0.6868      \\ \hline
Random Forest & 0.7298     & 0.6708       & 0.6737      & 0.7556        & 0.7174     & 0.6775      \\ \hline
LightGBM      & 0.7257     & 0.6769       & 0.6781      & 0.7481        & 0.7194     & 0.6946      \\ \hline
XGBoost       & 0.7272     & 0.6831       & 0.6601      & 0.7481        & 0.7217     & 0.6899      \\ \hline
\end{tabular}
\end{table}

==> sections/tables/super_park_not_in_test.tex <==
\begin{table*}
  \caption{The performance of various machine learning algorithms using  the Standard-features and Embedding-features on the Home-environment data as the test set. The models were trained on both Home-environment and Lab-environment data, but the performance metrics are calculated  on the Home-environment data only. The models using Standard-features perform better than their counterparts using Embedding-features in terms of both Binary Accuracy and AUC. \textcolor{orange}{Although the model's perform similarly in using the Standard-features, XGBoost outperforms others by considering both the AUC and Accuracy metrics}. However, the performance is slightly \st{lower}\textcolor{green}{worse} than the XGBoost model that uses both Home and Lab environment data in the test set: 0.0123 \textcolor{green}{decrease} in AUC and 0.004 \textcolor{green}{decrease} in Accuracy }
  \label{tab:res_super_park_not_in_test}
  \centering

\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Algorithm & \multicolumn{2}{|l|}{Standard-features} & \multicolumn{2}{|l|}{Embedding-features} \\ \hline
  & AUC  & Accuracy & AUC  & Accuracy \\\hline
 SVM & 0.7368  & 0.7336 & 0.7265  & 0.6964 \\
\hline
Random Forest  & 0.7317  & 0.7173 & 0.7194  & 0.7143 \\
\hline

LightGBM  & 0.7317 & 
0.7173 & 0.7327 & 0.6979 \\
\hline
XGBoost & \textbf{0.7379}  & \textbf{0.7366} & 0.7165  & 0.6949 \\
\hline

\end{tabular}

\end{table*}


% \begin{table*}
%   \caption{Results without SUPER-PARK in test-set}
%   \label{tab:res_super_park_not_in_test}
%   \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% Algorithm & \multicolumn{3}{|l|}{PRAAT} & \multicolumn{3}{|l|}{Max Little} & \multicolumn{3}{|l|}{Max Little + PRAAT} & \multicolumn{3}{|l|}{PASE} \\ \hline
%  & AUC & F1 & Acc. & AUC & F1 & Acc. & AUC & F1 & Acc. & AUC & F1 & Acc. \\\hline
% LightGBM & 0.6141 & 0.4449 & 0.625 & 0.7489 & 0.5548 & 0.7158 & 0.7317 & 0.5548 &
% 0.7173 & 0.7327 & 0.5522 & 0.6979 \\
% \hline
% XGBoost & 0.6121 & 0.4551 & 0.6116 & 0.7509 & 0.5898 & 0.7247 & 0.7379 & 0.5708 & 0.7366 & 0.7165 & 0.5393 & 0.6949 \\
% \hline
% SVM & 0.6651 & 0.5031 & 0.6786 & 0.7418 & 0.5901 & 0.7321 & 0.7368 & 0.5866 & 0.7336 & 0.7265 & 0.5737 & 0.6964 \\
% \hline
% Random Forest & 0.614 & 0.4515 & 0.6592 & 0.7387 & 0.5502 & 0.7202 & 0.7317 & 0.5548 & 0.7173 & 0.7194 & 0.5636 & 0.7143 \\
% \hline
% \end{tabular}
% }
% \end{table*}

==> sections/tables/super_park_not_in_training.tex <==
\begin{table*}
  \caption{The performance of various machine learning algorithms using  the Standard-features and Embedding-features on the Home-environment data. The SVM model using the Standard-features performs better than all other model combinations and the performance is quite similar to that of the previous models that uses both Home and lab environment data (Table ~\ref{tab:res_with_super_park}) }
  \label{tab:res_super_park_not_in_training}
  \centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Algorithm &  \multicolumn{2}{|l|}{Standard-features} & \multicolumn{2}{|l|}{Embedding-features} \\ \hline
  & AUC & Accuracy & AUC  & Accuracy \\\hline

SVM  & \textbf{0.7354}  & \textbf{0.7381} & 0.7288  & 0.6949 \\
\hline
Random Forest  & 0.7208  & 0.7188 & 0.7083  & 0.692 \\ \hline

LightGBM  & 0.7328  &
0.7158 & 0.7232  & 0.7054 \\
\hline
XGBoost  & 0.7326  & 0.7113 & 0.705  & 0.6935 \\

\hline
\end{tabular}

\end{table*}


% \begin{table*}
%   \caption{Results excluding SUPER PD from training}
%   \label{tab:res_super_park_not_in_training}
%   \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% Algorithm & \multicolumn{3}{|l|}{PRAAT} & \multicolumn{3}{|l|}{Max Little} & \multicolumn{3}{|l|}{Max Little + PRAAT} & \multicolumn{3}{|l|}{PASE} \\ \hline
%  & AUC & F1 & Acc. & AUC & F1 & Acc. & AUC & F1 & Acc. & AUC & F1 & Acc. \\\hline
% LightGBM & 0.606 & 0.4464 & 0.6429 & 0.7554 & 0.5872 & 0.7247 & 0.7328 & 0.5708 &
% 0.7158 & 0.7232 & 0.5459 & 0.7054 \\
% \hline
% XGBoost & 0.6125 & 0.4488 & 0.6235 & 0.7513 & 0.5796 & 0.7217 & 0.7326 & 0.5746 & 0.7113 & 0.705 & 0.5158 & 0.6935 \\
% \hline
% SVM & 0.6698 & 0.5214 & 0.683 & 0.7321 & 0.5905 & 0.7247 & 0.7354 & 0.574 & 0.7381 & 0.7288 & 0.6027 & 0.6949 \\
% \hline
% Random Forest & 0.6169 & 0.4316 & 0.6503 & 0.732 & 0.5321 & 0.7143 & 0.7208 & 0.5399 & 0.7188 & 0.7083 & 0.507 & 0.692 \\
% \hline
% \end{tabular}
% }
% \end{table*}
